Implicit Bias of SGD for Diagonal Linear Networks: a Provable Benefit of Stochasticity

Understanding the implicit bias of training algorithms is of crucial importance in order to explain the success of overparametrised neural networks. In this paper, we study the dynamics of stochastic gradient descent over diagonal linear networks through its continuous time version, namely stochastic gradient flow. We explicitly characterise the solution chosen by the stochastic flow and prove that it always enjoys better generalisation properties than that of gradient flow. Quite surprisingly, we show that the convergence speed of the training loss controls the magnitude of the biasing effect: the slower the convergence, the better the bias. To fully complete our analysis, we provide convergence guarantees for the dynamics. We also give experimental results which support our theoretical claims. Our findings highlight the fact that structured noise can induce better generalisation and they help explain the greater performances observed in practice of stochastic gradient descent over gradient descent.

==> Sections/checklist.tex <==
% !TeX root = ../main_implicit_bias_SGD.tex

%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See our main Theorem.}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss throughout the paper the limitations of our model.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See our different theorems and propositions.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See the Appendix.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Under figures.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{Everything runs on a laptop.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> Sections/conclusion.tex <==
% !TeX root = ../main_implicit_bias_SGD.tex

On the implicit bias: can we hope for a general effect with the loss ?

A study for sparcity  inducing problems : lasso, phase retrieval, matrix completion and factorisation. We can push it.


==> Sections/detailed_SDE_model.tex <==
% !TeX root = ../main_implicit_bias_SGD.tex

Continuous time modelling of sequential processes offer a large technical set of tools used to understand a dynamical system (think about derivatives!).  
It is often used to grasp the qualitative behaviour of the studied process (convergence, infinite time limit, invariants) or transfer directly the knowledge of continuous time quantities that help the analysis of the discrete time algorithm. A well-known example in optimisation is the use of continuous time limit dynamical system to help build Lyapunov functions. 
Indeed, a large part of the literature consider directly gradient flow to understand the implicit bias of gradient descent. 
Yet, when it comes to continuous time modelling, the first question we have to ask is whether the continuous time approximation is a reliable model of the algorithm. If we were to analyse gradient descent, then obviously, the corresponding gradient flow would be a good model. \Snote{$\beta^*$?}

\begin{equation}
    \label{eq:GF}
\begin{aligned}
\dd w_{t,+} &= - [X^\top  X (\beta_w - \beta^*)] \odot w_{t,+} \\
\dd w_{t,-} &= {\color{white} -} [X^\top  X (\beta_w - \beta^*)] \odot w_{t,-}.
\end{aligned}
\end{equation}

However, stochastic gradient descent is more challenging: even if in the limit of infinitesimal step-sizes, the noise does not play any role at first order, we would like to model SGD by a flow that takes into account its inherent noise. This can be done through adding a noise term to the gradient flow that allow basically to match the two first moments of the dynamics. This results in the following stochastic gradient flow (SGF):
%
\begin{equation}
    \label{eq:SGF}
\begin{aligned}
\dd w_{t,+} &= - [X^\top  X (\beta_w - \beta^*)] \odot w_{t,+}  + \sqrt{\gamma}\Sigma^{1/2}(w_t) \dd  B_t  \\
\dd w_{t,-} &= {\color{white} -} [X^\top  X (\beta_w - \beta^*)] \odot w_{t,-} - \sqrt{\gamma}\Sigma^{1/2}(w_t) \dd  B_t.
\end{aligned}
\end{equation}
%
where $\dd B_t$ is a Brownian on $\R^d$ and $\Sigma^{1/2}$ is any matrix $A$ such that to $A(w) A(w)^\top =  \Sigma(w) = \E_X\left[ \sigma_\mathrm{mul}(w)^{\otimes 2} | w \right]$ is the covariance noise of the stochastic gradient descent \note{define $\sigma_{mul}$ in previous section}. Note that we crucially modelled the noise on $w_+$  and $w_-$ with the same Brownian motion and structure as it is the case with the discrete algorithm. It is not the purpose of the paper to show consistency of this model in the small~$\gamma$ limit, but that it is a standard result of numerical approximation of SDE and has been done thoroughly in \cite{JMLR:v20:17-526}.

\paragraph*{Noise model.} One of the crux on the SDE modelling relies in the covariance of the noise $\Sigma(w)$. While many previous works model this covariance as an isotropic and state independent noise ($\Sigma = \sigma^2 I$), in a modern noiseless overparametrised framework, this does not make so much sense. Indeed, we would like to put emphasis on the fact that two features of the noise are particularly important. First, it is state-dependant and crucially cancels for an interpolator. Second, it has some geometric structure given by the architecture of the model, \emph{e.g} its rank is smaller that $n$ \note{to be  checked}. Guided by these two important properties, we will model the noise of our model in the following way:
%
\begin{align*}
\Sigma^{1/2}(w_t) \dd B_t = \sqrt{L(w_t)} w_t  \odot [X^\top \dd B'_t],
\end{align*}
%
where $\dd B'_t$ is a $\R^n$-Brownian motion. Indeed, to support our noise model, let us suppose that our features are generated by some Gaussian distribution of covariance $H \in \R^{d\times d}$. We know that for $n$ large enough, $X^\top X \sim H$: let us leverage this property to model the noise. Now, for $\eta = \beta - \beta_* $, 
%
\begin{align*}
\Sigma(w) = \E \left[ \sigma_\mathrm{mul}(w)^{\otimes 2} | w \right] &= \mathbb{E}_{\mathcal{N}(0, H) } [(X X^\top - x x^{\top}) \eta \eta^{\top} (X X^\top - x x^{\top}) \ | \ \eta ] \odot \left( w w^\top \right) \\
&\sim \left[\mathbb{E}_{\mathcal{N}(0, H) }( \langle x, \eta \eta^{\top} x \rangle x x^{\top} ) - H \eta \eta^{\top} H\right] \odot \left( w w^\top \right)  \\
&= \left[H \eta \eta^{\top} H + (\eta^{\top} H \eta) H \right] \odot (w w^\top)\\
&\sim  L(w) \left(X^\top X\right) \odot \left( w w^\top \right) \\
&= L(w) \left(\diag(w) X^\top\right)\left(\diag(w) X^\top\right)^\top  .
\end{align*}
%
Once again, note that we are interested in \emph{modelling} the noise covariance, that is, finding its structure and scale, hence, a low concern about small deviations to it and constant. We expect the mixing properties of the Gaussian distribution to hold for a large class of distribution of interest. 
%
\paragraph*{Stochastic gradient flow.} We can rewrite the stochastic gradient flow with the proper noise model:
%
\begin{equation}
\begin{aligned}
\dd w_{t,+} &= - [X^\top  X (\beta_w - \beta^*)] \odot w_{t,+}  + \sqrt{\gamma} L (w_t)^{1/2} w_{t,+} \odot [X^\top \dd  B_t]  \\
\dd w_{t,-} &= {\color{white} -} [X^\top  X (\beta_w - \beta^*)] \odot w_{t,-} - \sqrt{\gamma} L (w_t)^{1/2} w_{t,-} \odot [X^\top \dd  B_t].
\end{aligned}
\end{equation}

%
Recall that, as importantly remarked in \cite{wojtowytsch2021stochastic} the noise in our continuous time model is consistent with the one of SGD: it is low-rank and scales with the loss at time~$t$. This stochastic differential equation is the starting point of the analysis of this paper.







==> Sections/old_implicit_bias.tex <==
Now that the setting and the algorithm which we consider are clearly defined, we will give our main theorem. 
Beforehand we introduce a potential function $\phi_\alpha$ which 
will appear in roughly all our results. 


\begin{definition}
\label{def:potential_function}
    For $0 < \alpha \in \R^d$, let $\phi_\alpha : \R^d \to \R $ such that 
\begin{align}
\label{eq:potential_function}
    \phi_\alpha (\beta) = \frac{1}{4} \big[  \sum_{i = 1}^d \beta_i \arcsinh(\frac{\beta_i}{2 \alpha_i^2}) - \sqrt{\beta_i^2 + 4 \alpha_i^4} \big ] .
\end{align}
    By abuse of notation, for $\alpha \in \R$ we will write $\phi_{\alpha} = \phi_{\alpha \mathbf{1}}$.
\end{definition}

% For reasons which will soon become clear, we call our function $\phi_\alpha$ our potential. 

Though this potential has a non-trivial expression, we point out the following two simple asymptotic behaviours 
for fixed $\beta \in \R^d$:
$\phi_\alpha(\beta) \underset{\alpha \to 0}{\sim} \frac{1}{2} \ln \big( \frac{1}{\alpha} \big ) \Vert \beta \Vert_1$ and
$\phi_\alpha(\beta) \underset{\alpha \to + \infty}{=} 2 \alpha^2 + \frac{1}{4 \alpha^2}  \Vert \beta \Vert_2^2 + o(\alpha^{-2})$.
Hence $\phi_\alpha$ resembles the $\ell_1$ norm for small values of $\alpha$ and the squared $\ell_2$ norm 
for large values. 
 
We now state our main theorem \Snote{remarque Loucas $\alpha^2 <-> \alpha^2 d$ } .

\begin{thm}
\label{thm:main_theorem}
Let $\beta^*_{\ell_1} = \underset{\beta \in \R^d \ \text{s.t.} \ X \beta = y}{ \argmin } \Vert \beta \Vert_1$. 
For $ p \leq \frac{1}{2}$ and $w_0 = \alpha  \mathbf{1} \in \R^{2d}$
assume that
\begin{equation}
    \label{ineq:gamma_upperbound}
\gamma \leq \frac{1}{330 \ln \big( \frac{2}{p} \big ) \lambda_{max} (X X^{\top}) \max{ \Big \{  \Vert \beta^*_{\ell_1} \Vert_1 } \ln \big( \sqrt{2} 
    \frac{ \Vert \beta^*_{\ell_1}  \Vert_1}{\alpha^2} \big), \alpha^2 d \Big \} } ,
\end{equation}
then with probability at least $1-p$, the stochastic gradient flow $(w_t)_{t \geq 0}$ converges 
and the corresponding flow $(\beta_t)_{t \geq 0}$ converges towards a zero-training error solution $\beta_{\infty}$ 
which verifies
\begin{equation}
\label{eq:main_theorem_min_prob}
        \beta_{\infty} = \underset{\beta \in \R^d}{ \mathrm{arg \ min \ }} \phi_{\alpha_{\eff}}(\beta) \quad \text{such that } \quad X \beta = y,
\end{equation}
where $\alpha_{\eff} = \alpha \ \exp \Big( -\frac{\gamma}{2} \diag(H) \int_0^{+ \infty} L(\beta_s) \diff s \Big) \in \R^d$.
\end{thm}


Our theorem is three-fold: with high probability and for an adequate choice of step size $\gamma$, 
(1) the flow $(\beta_t)_{t \geq 0}$ converges, 
(2) $\beta_\infty$ is an interpolating solution, i.e. $X \beta_\infty = y$ ,
(3) this solution minimises a particular potential which depends on explicit features of the dynamics.
Note that the minimisation problem~\ref{eq:main_theorem_min_prob} only makes sense \textit{a posteriori} since the 
quantity $\alpha_\eff$ depends on the whole stochastic trajectory.
Concerning the convergence result, notice that it holds even though the step size $\gamma$ is constant. 
This is not illogical since we assume that the noise vanishes at the optimum. 
The upperbound on the maximal value of $\gamma$ in \ref{ineq:gamma_upperbound} has a classical dependence
on $\lambda_{max}(X X^{\top})$ which can be computed, but also on the unknown value of $\Vert \beta^*_{l_1} \Vert_1$.
However in practice we choose the highest value of $\gamma$ for which the iterates converge.
% we will see that this strategy makes sense in our framework since it will lead to the best implicit bias. 
Regarding the magnitude of $\alpha^2 d$, note that it corresponds to the $\ell_2$ norm of the weights' initialisation: $\Vert w_{t = 0} \Vert_2^2 = 2 \alpha^2 d$. 
Therefore in practice and even in high dimension, 
 $\alpha^2 d$ is roughly equal to $1$ and therefore $\alpha^2 d \ll \Vert \betasparse \Vert_1$.
Also we believe that the $\ln \big(  \frac{\Vert \beta^* \Vert_1}{\alpha^2} \big)$ factor in the upperbound
\ref{ineq:gamma_upperbound} is an artefact of our analysis 
and a finer analysis could get rid of it. 
% The constant $330$ is non-informative and a more careful analysis could probably lower it down.
It is hence best to think of the upperbound on $\gamma$ to simply be $\gamma \leq O( \frac{1}{\lambda_{max} \Vert \beta^* \Vert_1 })$.

The most remarkable aspect of our result is that the recovered solution $\beta_\infty$ minimises a potential which depends on an effective 
parameter $\alpha_{\eff} < \alpha \mathbf{1}$. Note that this parameter is in $\R^d$, and following our previous remark,
 the smaller its values and the closer the potential is to the $\ell_1$ norm. 
This effective parameter is controlled by the loss integral $\int_0^{+ \infty} L(\beta_s) \diff s$: the higher the integral and the smaller the 
effective initialisation scale. In other words, the slower the loss converges to $0$, the "richer" the implicit bias. We point 
out that the value of this integral still depends on $\gamma$ and $\alpha$, this dependency will be made clear in the next section.
According to our result and in order to improve the implicit bias, one can either decrease the initialisation scale $\alpha$, or
try to "slow down" the convergence. We will see that adding artificial label noise does just that.
However it must be kept in mind that, as explained in Srebro et al., there is a tension between generalisation and optimisation: a 
longer training time might improve generalisation but comes at the cost of... a longer training time. However it is clear experimentally that
SGD systematically wins the tradeoff over GD.

Though it is less our focus, our result still holds as $\alpha \to +\infty$ which corresponds to the kernel regime. In this regime we show 
in the appendix that $\int_0^{+ \infty} L(\beta_s) ds \underset{\alpha \to \infty}{\to} 0$ and hence SGF and GF converge towards the same solution. However in 
this case we need infinitely small $\gamma$ to ensure convergence.
\Snote{comment: $\diag H$, no speed of convergence}

\paragraph{Sketch of proof.} The hardest part of this result is to show the convergence of the flow with high probability.
However once the convergence is shown, describing the minimisation problem 
the solution $\beta_\infty$ minimises is straightforward.
In the following section we give several properties which constitute the major keys of the proof of our theorem.

% the iterates $(\beta_t)_{t \geq 0}$ follow a "continuous time-varying potential mirror descent". In this framework, similarly
% to the classical mirror descent framework, it is easy 
% to describe the resulting implicit bias. Showing the convergence of the flow is more tricky, to do so we consider an adequate
% Lyapunov function. This analysis also enables to control several dynamical quantities, which we give in the following section.

%  they key element which controls the final implicit 
% bias (apart from the initialisation scale $\alpha$) is the quantity $\int_0^{+ \infty} L(\beta_s) ds$. This
% quantity basically represents the speed at which the training error goes to $0$.
% The higher this integral, the smaller the $\alpha_{eff}$ and the "richer" the implicit bias.


% \Snote{

% \begin{itemize}
    % \item our theorem is threefold: convergence, towards an interpolator and characterisation of the solution.
    % \item The slower the loss converges to $0$, the bigger the value of $\int_0^{+ \infty} L(\beta_s) ds$ and the smaller 
% the effective scale of $\alpha$.
%  \item $\diag H$ appears and not the eigenvalues, this makes sense because because ... 
%  \item note that because of the stochasticity of the brownian motion we can only expect a results in high probability
%  \item the condition over $\gamma$ is necessary in order to ensure high probability convergence of the gradient flow. 
%  However it is not necessary, once convergence is assumed, to characterise the implicit bias. As explained in the informal theorem statement. 
%  As soon as convergence of the gradient flow is assured, the implicit bias follows
% \item note that the value of $\alpha^2 d$ corresponds to the $\ell_2$ norm of the weight initialisation: $\Vert w(t = 0) \Vert_2^2 = 2 \alpha^2 d$. Hence even if $d$ is big, 
% in practice $\alpha^2 d$ is chosen to roughly be equal to $O(1)$.
% \item We believe that the $\ln \big(  \frac{\Vert \beta^* \Vert_1}{\alpha^2} \big)$ is a by-product of our analyis and should not be there. 
% \item Regarding the last two remarks it is hence best to think of the condition over $\gamma$ to simply be $\gamma \leq O( \frac{1}{\lambda_{max} \Vert \beta^* \Vert_1 })$.
% \item  Description of the dynamics are also provided in the next section.
% \item Speed of convergence is missing, we cannot directly compare GF and SGF and state that SGF is better. To claim superiority we need to take into account speed of convergence, 
% not necessarily of loss but of iterates.
% \item According to the theorem, in order to improve the implicit bias, one can either decrease the initialisation scale $\alpha$, or one can try and "slow done" the convergence.
% We will see that adding artificial label noise does so.
% \item In the next section we show that the SGF follows an "online continuous time-varying mirror descent".
% \item result still holds for $\gamma \to \infty$, which corresponds to the kernel regime. However in this case we need 
% infinitely small step sizes for convergence. 
% \item keep in mind that $\int_0^{+ \infty} L(\beta_s) ds$ still depends on $\gamma$ and on $\alpha$.
% \item comment on fixed step size.
% \end{itemize}

%     Note that in all case $\alpha_{\eff} < \alpha$. Our result clearly shows that the slower the loss converges,
% the better the implicit bias will be. By better we mean that the bound on the $\ell_1$ norm will be better.





% Again : kind of time dependent mirror descent Gives the result as in Srebro and al. (at the end of the day, this is the only to really identify the implicit bias).

% Shape of the implicit bias.

% Use previous result to give the scale of loss integral

% Plots and order of magnitude.

% Interpretations : 

% \begin{itemize}

% \item Talk about step size droping effect.

% \item Add label noise. Plots.

% \item Show the $2-d$ plots of Scott.

% \item Do we have a principled interpretation ? Wind, Tequila, dream exploration.


% \end{itemize}

% }
